Renormalisation of Fermionic Cellular Automata

We present an exact renormalisation scheme for fermionic cellular automata on hypercubic lattices. By grouping neighbouring cells into tiles and selecting subspaces within them, multiple evolution steps on the original system correspond to a single step of an effective automaton acting on the subspaces. We derive a necessary and sufficient condition for renormalisability and fully characterise the renormalisation flow for two-cell tiles and two time steps of nearest-neighbour fermionic automata on a chain of spinless modes, identifying all fixed points.

==> Renormalisation_of_fermionic_cellular_automata/figures/LocUnitprim.tikz.tex <==
\begin{tikzpicture}
\foreach \t in  {0,...,2}{
\draw[black]  (\bitdistance*\t+1.5*\bitsize*\t,3*\hdist) -- (\bitdistance*\t+1.5*\bitsize*\t, \bitsize*0.5+2pt) ;
\node at (\bitdistance*\t+1.5*\bitsize*\t,-0.1) {\t}; 
}
\foreach \t in {0,...,2}{
\node[U] at (1.5*\bitsize*\t+\bitdistance*\t,0.0001*\hdist) {$\mathcal U'$};
}

\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/M1.tikz.tex <==
\begin{tikzpicture}
\draw[black]  (\bitdistance+\bitsize,1)--(\bitdistance+\bitsize,-1);
\draw[black]  (0,1)--(0,-1);
\node[M1] at (\bitsize+\transfoffset,0) {$\mathcal{M}_1$};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/M1prim.tikz.tex <==
\begin{tikzpicture}
\draw[black]  (\bitdistance+\bitsize,1)--(\bitdistance+\bitsize,-1);
\draw[black]  (0,1)--(0,-1);
\node[M1] at (\bitsize+\transfoffset,0) {$M_1'$};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/M1unit.tikz.tex <==
\begin{tikzpicture}
\foreach \t in {0,...,5}{
\draw[black]  (\t*\bitdistance+\t*\bitsize,1)--(\t*\bitdistance+\t*\bitsize,-1);
}
\foreach \t in {0,...,2}{
\node[U] at (\bitdistance*\t*2+\bitsize*\t*2,0) {$U$};
\node[U] at (\bitsize+\bitdistance+\bitdistance*\t*2+\bitsize*\t*2,0) {$V$};
}
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/M2.tikz.tex <==
\begin{tikzpicture}
\draw[black]  (\bitdistance+\bitsize,-1)--(\bitdistance+\bitsize,1);
\draw[black]  (0,-1)--(0,1);
\node[M2] at (\bitsize+\transfoffset,0) {$\mathcal{M}_2$};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/M2qbit.tikz.tex <==
\begin{tikzpicture}
\draw[black]  (\bitdistance+\bitsize,1.5)--(\bitdistance+\bitsize,-1);
\draw[black]  (0,1.5)--(0,-1);
\node[Cif] at (\bitsize+\transfoffset,0) {$\mathcal{C}_\phi$};
\node[U] at (0,\hdist*0.5) {$\mathcal{U}$};
\node[U] at (\bitdistance+\bitsize,\hdist*0.5) {$\mathcal{U}$};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/TnPiZen.tikz.tex <==
\begin{tikzpicture}[baseline=(O.base)]
\node (O) at (0,0.25*\hdist) {};
\foreach \t in  {0,...,1}{
\draw[black]  (\bitdistance*\t+\bitsize*\t,3*\hdist) -- (\bitdistance*\t+\bitsize*\t, \bitsize*0.5+2pt) ;
}
\node[bit]  at (0,0)   {\tiny$\Pi_0$};
\node[bit] at (\bitdistance+\bitsize,0) {\tiny $\Pi_{\mathcal{M}}$};
\node[U] at (\bitsize+\bitdistance,\hdist) {$\mathcal{Z}^\dag$};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/TnPish.tikz.tex <==
\begin{tikzpicture}[baseline=(O.base)]
\node (O) at (0,0.25*\hdist) {};
\foreach \t in  {0,...,1}{
\draw[black]  (\bitdistance*\t+\bitsize*\t,3*\hdist) -- (\bitdistance*\t+\bitsize*\t, \bitsize*0.5+2pt) ;
}
\node[bit]  at (0,0)   {\tiny $\Pi_0$};
\node[bit] at (\bitdistance+\bitsize,0) {\tiny $\Pi_{\mathcal{M}}$};
\node[M2] at (\bitsize+\transfoffset,\hdist) {$\mathcal{U}$};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/Ucirc.tikz.tex <==
\begin{tikzpicture}
\foreach \t in {0,...,3}{
\draw (\bitsize*\t+\bitdistance*\t,-1)--(\bitsize*\t+\bitdistance*\t,1);
\node[U] at (\bitsize*\t+\bitdistance*\t,0) {$U$};
}
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/Uprimeswap.tikz.tex <==
\begin{tikzpicture}
\foreach \t in  {0,1}{
\draw[black]  (\bitdistance*\t+\bitsize*\t,0) -- (\bitdistance*\t+\bitsize*\t, 1.5*\hdist) ;
\node[U]  at (\bitdistance*\t+\bitsize*\t,0.25*\hdist)   {$U'$};
}
\draw[black]  (0,1*\nhdist) -- (\bitdistance+\bitsize,0) ;
\draw[black]  (0,0) -- (\bitdistance+\bitsize,1*\nhdist) ;
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/metatikz.tex <==
\usetikzlibrary {arrows.meta}
\usetikzlibrary{%
    decorations.pathreplacing,%
    decorations.pathmorphing,%
    arrows,
    arrows.meta,
    positioning,
    calc,
    shapes,
    shadows,
    shapes.geometric
    }

\definecolor{myblue1}{RGB}{0,157,209}

\tikzset{
  local/.style 2 args={
    rectangle, 
    rounded corners=1pt, 
    minimum height={#1},
    minimum width={#2},
    align=center, 
    line width=1pt,
    draw=white,
    opacity=0.7,
    font=\color{black}\sffamily, 
    fill=myblue1
  },
  local/.default={0.6 cm}{0.6 cm},
  T/.style={
 	rectangle,
 	rounded corners=1pt ,
 	align=center,
 	line width =2pt,
 	draw=black,
 	opacity=0.7,
    font=\color{black}\sffamily, 
    fill=myblue1
  }
 }

==> Renormalisation_of_fermionic_cellular_automata/figures/tildeLR.tikz.tex <==
\begin{tikzpicture}[baseline=(O.base)]
\node (O) at (0,0) {};
\node[LR] at (\bitsize+\transfoffset,0) {\LRtilde};
\node[LR] at (\bitsize+\transfoffset+\transfdistance,0) {\LtilR};
\end{tikzpicture}

==> Renormalisation_of_fermionic_cellular_automata/figures/twocells.tikz.tex <==
\begin{tikzpicture}
\foreach \a in {0,...,1}{
\node[bit] (A\a ) at (\a cm,0) {};
\node at ($(A\a)-(0,1)$) {\a};
}

\end{tikzpicture}


==> Renormalisation_of_fermionic_cellular_automata/tikzstyle.tex <==
\usetikzlibrary {arrows.meta}
\usetikzlibrary{%
    decorations.pathreplacing,%
    decorations.pathmorphing,%
    arrows,
    arrows.meta,
    positioning,
    calc,
    shapes,
    shadows,
    shapes.geometric,
   math
    }

\definecolor{myblue1}{HTML}{3A9831}
\definecolor{myblue2}{HTML}{08543A}
\definecolor{mycolor}{HTML}{FFC56E}
\definecolor{cifcolor}{HTML}{D50032}
\definecolor{Mswapcolor}{HTML}{FF571F}
\definecolor{Ucolor}{HTML}{C4D600}
\definecolor{phasecolor}{HTML}{FE5000}
\definecolor{phasecolorbis}{HTML}{C8102E}
\definecolor{phasecolortris}{HTML}{EAAA00}
\definecolor{tassellationcol}{HTML}{E4CC00}
\definecolor{important}{HTML}{E55121}
\definecolor{bluenonren}{rgb}{0.21,0.48,0.80}
\definecolor{blueren}{RGB}{166, 216, 236}
\newcommand\bitsize{0.6 cm}
\newcommand\projspace{0.12cm}
\def\LR{\hspace{\projspace}$\m{L}$\hspace{\projspace} \nodepart{two}\hspace{\projspace}$\m{R}$\hspace{\projspace}}
\def\LRtil{\hspace{\projspace}$\tilde{\m{L}}$\hspace{\projspace} \nodepart{two}\hspace{\projspace}$\tilde{\m{R}}$\hspace{\projspace}}
\def\LRbar{\hspace{\projspace}$\bar{\m{L}}$\hspace{\projspace} \nodepart{two}\hspace{\projspace}$\bar{ \m{R}}$\hspace{\projspace}}
\def\LtilR{\hspace{\projspace}$\tilde{\m{L}}$\hspace{\projspace} \nodepart{two}\hspace{\projspace}$\m{R}$\hspace{\projspace}}
\def\LRtilde{\hspace{\projspace}${\m{L}}$\hspace{\projspace} \nodepart{two}\hspace{\projspace}$\tilde{\m{R}}$\hspace{\projspace}}
\newcommand\bitdistance{1 cm}
\newcommand\transfborder{0.1cm}
\newcommand\transfsize{\bitsize+\bitdistance-\transfborder}
\tikzmath{
\transfdistance=2*\bitdistance +2*\bitsize;
}
\tikzmath{
\transfoffset= 0.25*\bitdistance - \transfborder*0.5;
\halfsize=\bitsize*0.5;
\halfdistance=\bitdistance*0.5;
}
\newcommand\hdist{\bitsize+\bitdistance+\halfsize}
\newcommand\nhdist{-\bitsize-\bitdistance-\halfsize}
\newcommand\halfleft{-\bitsize-\transfoffset + \transfsize*0.5-\transfborder}
\tikzset{
  local/.style 2 args={
    rectangle, 
    rounded corners=10pt, 
    minimum height={#1},
    minimum width={#2},
    align=center, 
    line width=1pt,
    draw=white,
    font=\color{black}\sffamily, 
    fill=myblue1
  },
  local/.default={0.6 cm}{0.6 cm},
  M1/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={#1},
   	 minimum width={#2},
 	line width =1pt,
 	draw=black,
    font=\color{black}\sffamily, 
    fill=myblue1,
  },
  M1/.default={\bitsize}{\transfsize},
 M2/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={#1},
   	 minimum width={#2},
 	line width =1pt,
 	draw=black,
    font=\color{black}\sffamily, 
    fill=myblue2
  },
  M2/.default={\bitsize}{\transfsize},
 G/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={#1},
   	 minimum width={#2},
 	line width =1pt,
 	draw=black,
    font=\color{black}\sffamily, 
    fill=mycolor
  },
  G/.default={\bitsize}{\transfsize},
  bit/.style 2 args= {  
    rectangle, 
    rounded corners=10pt, 
    minimum height={#1},
    minimum width={#2},
    align=center, 
    line width=1pt,
    draw=black,
    font=\color{black}\sffamily, 
    fill=White
   },
 bit/.default={\bitsize}{\bitsize},
 bittil/.style 2 args= {  
    rectangle, 
    rounded corners=10pt,
    drop shadow, 
    minimum height={#1},
    minimum width={#1},
    align=center, 
    line width=1pt,
    draw=black,
    font=\color{black}\sffamily, 
    fill={#2}
   },
 tassel/.style 2 args= {  
    rectangle, 
    rounded corners=10pt,
    minimum height={#1},
    minimum width={#1},
    align=center, 
    line width=1pt,
    opacity={#2},
    draw=black,
    font=\color{black}\sffamily, 
    fill=tassellationcol
   },
  U/.style= {  
    rectangle, 
    rounded corners=7pt, 
    minimum height={\bitsize},
    minimum width={\bitsize},
    align=center, 
    line width=1pt,
    draw=black,
    fill=Ucolor,
    font=\color{black}\sffamily, 
   },
  LRbit/.style = {  
    rectangle, 
    rounded corners=10pt, 
    minimum height={\bitsize},
    minimum width={\transfsize},
    align=center, 
    line width=1pt,
    draw=black,
    fill=gray,
    font=\color{black}\sffamily, 
   },
   pi/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={#1},
   	 minimum width={#2},
 	line width =1pt,
 	draw=black,
	opacity=1,
    font=\color{black}\sffamily, 
    fill=yellow,
  },
  pi/.default={\bitsize}{\transfsize},
%LR/.style  2 args={
 %	rectangle split,
%	rectangle split horizontal,
%	rectangle split parts=2,
% 	rounded corners=2pt ,
% 	align=center,
% 	minimum height={#1},
  % 	 minimum width ={#2},
% 	line width =1pt,
% 	draw=black,
%	opacity=0.6,
 %   font=\color{black}\sffamily, 
 %   fill=yellow,
 % },
%LR/.default={\bitsize}{\transfsize},
LR/.style ={
 	rectangle split,
	minimum height=0.6 cm,
   	minimum width =7.5cm,
	rectangle split horizontal,
	rectangle split parts=2,
 	rounded corners=10pt ,
 	align=center,
 	line width =1pt,
 	draw=black,
	opacity=1,
    font=\color{black}\sffamily, 
    fill=yellow,
 	text centered,
  },
  swap/.pic ={
	\draw (-\bitdistance,-1)--(-\bitdistance,-0.75)--(\bitdistance,0.75)--(\bitdistance,1);
	\draw (\bitdistance,-1)--(\bitdistance,-0.75)--(-\bitdistance,0.75)--(-\bitdistance,1);  
%  \draw (-\halfsize-\halfdistance,\nhdist*0.5) -- (-\halfsize-\halfdistance,\nhdist*0.25) -- (\halfsize+\halfdistance,\hdist*0.25) -- (\halfsize+\halfdistance,\hdist*0.5);
   % \draw (\halfsize+\halfdistance,\nhdist*0.5) -- (\halfsize+\halfdistance,\nhdist*0.25) -- (-\halfsize-\halfdistance,\hdist*0.25) -- (-\halfsize-\halfdistance,\hdist*0.5);
  },
Cif/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={#1},
   	 minimum width={#2},
 	line width =1pt,
 	draw=black,
    font=\color{black}\sffamily, 
    fill=cifcolor
  },
Cif/.default={\bitsize}{\transfsize},
Mswap/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={#1},
   	 minimum width={#2},
 	line width =1pt,
 	draw=black,
    font=\color{black}\sffamily, 
    fill=Mswapcolor
  },
  Mswap/.default={\bitsize}{\transfsize},
phase/.style 2 args={
 	rectangle,
 	rounded corners=10pt ,
 	align=center,
 	minimum height={\bitsize},
   	 minimum width={#1},
 	line width =1pt,
 	draw=black,
    font=\color{black}\sffamily, 
    fill={#2}
  },
Op/.style 2 args={
	circle,
	draw=black,
	line width=1pt,
	font=\color{black}\sffamily ,
	minimum height={#1},
   	 minimum width={#2},
   	 fill=White,
 },
 Op/.default={\bitsize*0.25}{\bitsize*0.25},
 J/.pic={
  \draw (-\bitdistance,\nhdist)--(0,\nhdist*0.5)--(\bitdistance,\nhdist),},
 }

==> figures/M1prim.tikz.tex <==
\begin{tikzpicture}
\draw[black]  (\bitdistance+\bitsize,1)--(\bitdistance+\bitsize,-1);
\draw[black]  (0,1)--(0,-1);
\node[M1] at (\bitsize+\transfoffset,0) {$M_1'$};
\end{tikzpicture}

==> figures/M1unit.tikz.tex <==
\begin{tikzpicture}
\foreach \t in {0,...,5}{
\draw[black]  (\t*\bitdistance+\t*\bitsize,1)--(\t*\bitdistance+\t*\bitsize,-1);
}
\foreach \t in {0,...,2}{
\node[U] at (\bitdistance*\t*2+\bitsize*\t*2,0) {$U$};
\node[U] at (\bitsize+\bitdistance+\bitdistance*\t*2+\bitsize*\t*2,0) {$V$};
}
\end{tikzpicture}

==> figures/Ucirc.tikz.tex <==
\begin{tikzpicture}
\foreach \t in {0,...,3}{
\draw (\bitsize*\t+\bitdistance*\t,-1)--(\bitsize*\t+\bitdistance*\t,1);
\node[U] at (\bitsize*\t+\bitdistance*\t,0) {$U$};
}
\end{tikzpicture}

==> figures/Uprimeswap.tikz.tex <==
\begin{tikzpicture}
\foreach \t in  {0,1}{
\draw[black]  (\bitdistance*\t+\bitsize*\t,0) -- (\bitdistance*\t+\bitsize*\t, 1.5*\hdist) ;
\node[U]  at (\bitdistance*\t+\bitsize*\t,0.25*\hdist)   {$U'$};
}
\draw[black]  (0,1*\nhdist) -- (\bitdistance+\bitsize,0) ;
\draw[black]  (0,0) -- (\bitdistance+\bitsize,1*\nhdist) ;
\end{tikzpicture}

==> figures/metatikz.tex <==
\usetikzlibrary {arrows.meta}
\usetikzlibrary{%
    decorations.pathreplacing,%
    decorations.pathmorphing,%
    arrows,
    arrows.meta,
    positioning,
    calc,
    shapes,
    shadows,
    shapes.geometric
    }

\definecolor{myblue1}{RGB}{0,157,209}

\tikzset{
  local/.style 2 args={
    rectangle, 
    rounded corners=1pt, 
    minimum height={#1},
    minimum width={#2},
    align=center, 
    line width=1pt,
    draw=white,
    opacity=0.7,
    font=\color{black}\sffamily, 
    fill=myblue1
  },
  local/.default={0.6 cm}{0.6 cm},
  T/.style={
 	rectangle,
 	rounded corners=1pt ,
 	align=center,
 	line width =2pt,
 	draw=black,
 	opacity=0.7,
    font=\color{black}\sffamily, 
    fill=myblue1
  }
 }

==> figures/tildeLR.tikz.tex <==
\begin{tikzpicture}[baseline=(O.base)]
\node (O) at (0,0) {};
\node[LR] at (\bitsize+\transfoffset,0) {\LRtilde};
\node[LR] at (\bitsize+\transfoffset+\transfdistance,0) {\LtilR};
\end{tikzpicture}

==> figures/twocells.tikz.tex <==
\begin{tikzpicture}
\foreach \a in {0,...,1}{
\node[bit] (A\a ) at (\a cm,0) {};
\node at ($(A\a)-(0,1)$) {\a};
}

\end{tikzpicture}

